Calibration of Advanced Virgo and reconstruction of detector strain h(t) during the Observing Run O3

The three Advanced Virgo and LIGO gravitational wave detectors participated to the third observing run (O3) between 1 April 2019 15:00 UTC and 27 March 2020 17:00 UTC,leading to several gravitational wave detections per month. This paper describes the Advanced Virgo detector calibration and the reconstruction of the detector strain $h(t)$ during O3, as well as the estimation of the associated uncertainties. For the first time, the photon calibration technique as been used as reference for Virgo calibration, which allowed to cross-calibrate the strain amplitude of the Virgo and LIGO detectors. The previous reference, so-called free swinging Michelson technique, has still been used but as an independent cross-check. $h(t)$ reconstruction and noise subtraction were processed online, with good enough quality to prevent the need for offline reprocessing, except for the two last weeks of September 2019. The uncertainties for the reconstructed $h(t)$ strain, estimated in this paper in a 20-2000~Hz frequency band, are frequency independent: 5% in amplitude, 35 mrad in phase and 10 $\mu$s in timing, with the exception of larger uncertainties around 50 Hz.

==> definitions.tex <==

\RequirePackage{xspace}

%\newcommand{\dv}[1]{{\color{magenta} Didier: #1}}
%\newcommand{\lr}[1]{{\color{blue} Loic: #1}}
%\newcommand{\msa}[1]{{\color{orange} Monica: #1}}

%\newcommand{\dv}[1]{{\color{blue} #1}}
%\newcommand{\lr}[1]{{\color{blue} #1}}
%\newcommand{\msa}[1]{{\color{blue} #1}}

\newcommand{\dv}[1]{ #1}
\newcommand{\lr}[1]{ #1}
\newcommand{\msa}[1]{ #1}
%
\newcommand{\de}[1]{{\color{darkgreen} Dimitri: #1}}
\newcommand{\paul}[1]{{\color{cyan} Paul: #1}}
\newcommand{\todo}[1]{{\color{red} TO-DO: #1}}
\newcommand*\rot{\rotatebox{90}} 

\newcommand{\dg}{\ensuremath{^\circ}}
\newcommand{\VIRGO}{\small VIRGO}
\newcommand{\RMS}{{\small RMS}}
\newcommand{\RMSs}{{\small RMS}s}
\newcommand{\ADC}{{\small ADC}}
\newcommand{\ADCs}{{\small ADC}s}
\newcommand{\DAC}{{\small DAC}}
\newcommand{\DACs}{{\small DAC}s}
\newcommand{\GW}{GW}
\newcommand{\GWs}{GWs}
\newcommand{\ITF}{ITF}
\newcommand{\TF}{TF}
\newcommand{\TFs}{TFs}
\newcommand{\FFT}{FFT}
\newcommand{\FFTs}{FFTs}
\newcommand{\HP}{HP}
\newcommand{\LN}{LN}
\newcommand{\DSP}{DSP}
\newcommand{\DSPs}{DSPs}
\newcommand{\NE}{NE}
\newcommand{\NI}{NI}
\newcommand{\WE}{WE}
\newcommand{\WI}{WI}
\newcommand{\BS}{BS}
%\newcommand{\PR}{PR}
\newcommand{\TEMOO}{$\mathrm{TEM_{00}}$}
\newcommand{\mus}  {$\upmu \text{s}$}
\newcommand{\mum}  {$\upmu \text{m}$}
\newcommand{\murad}{$\upmu \text{rad}$}

\newcommand{\PrBACp}{$\mathrm{Pr\_B1\_ACp}$}
\newcommand{\prl}{Phys. Rev. Letters}
\newcommand{\SczCorr}{$\mathrm{Sc\_*\_zCorr}$}
\newcommand\rednote[1]{\textcolor{red}{\bf {#1}}}
\newcommand\bluenote[1]{\textcolor{blue}{\bf {#1}}}

\newcommand{\VirgoAcronym}[3]{ \noindent {\bf #1}: {\it #2}, #3. \\}
\newcommand{\VirgoAcronymShort}[2]{ \noindent {\bf #1}: #2. \\}

